ZipperChain: Transmuting Trusted Third-Party Services Into Trustless Atomic Broadcast

Distributed ledger technologies (DLTs) rely on distributed consensus mechanisms to reach agreement over the order of transactions and to provide immutability and availability of transaction data. Distributed consensus suffers from performance limitations of network communication between participating nodes. BLOCKY ZipperChain guarantees immutability, agreement, and availability of transaction data, but without relying on distributed consensus. Instead, its construction process transfers trust from widely-used, third-party services onto ZipperChains's correctness guarantees. ZipperChain blocks are built by a pipeline of specialized services deployed on a small number of nodes connected by a fast data center network. As a result, ZipperChain transaction throughput approaches network line speeds and block finality is on the order of 500 ms. Finally, ZipperChain infrastructure creates blocks centrally and so does not need a native token to incentivize a community of verifiers.

==> appendices/VPBS_and_other_old_stuff.tex <==


% The goal of \sol\ is to provide correctness guarantees on par with other blockchain implementations, namely \emph{immutability}, \emph{agreement}, and \emph{availability}.
% While there exists a considerable variety in blockchain protocols, for many we can define the state of a blockchain as a totally ordered ledger of transactions.
% Any node may execute these transactions in that order to obtain a key-value store representing the values of token accounts and smart contract variables.
% This perspective on blockchains allows us to specify the correctness guarantees as follows:
% \begin{itemize}
%     \item \textbf{Blockchain-Immutability} -- If a valid quorum node has a transaction at some position in its ledger, it will continue to have that transaction at that position in its ledger.
%     \item \textbf{Blockchain-Agreement} -- If a valid quorum node has a transaction at some position in its ledger, all valid quorum nodes will have that transaction at that position and only that position in their ledgers.
%     \item \textbf{Blockchain-Availability} -- The quorum of valid nodes remains valid.
%     % , which implies that all nodes are never replaced simultaneously, which allows the state to persist...
% \end{itemize}
% Note that Blockchain-Availability implies that all nodes of a quorum are never replaced simultaneously, which allows the state of the blockchain to persist.
% Additionally, Blockchain-Availability may also be considered to provide liveness, where, barring network partitions, a user may always write to and read transactions from the blockchain.
% Finally, the quorum in many blockchains is a qualified majority.

% \begin{table}[h]
%     \centering
%     \begin{tabular}{l|l}
%     \hline
%     Symbol & Meaning \\
%     \hline
%      $\val$ & Consensus value \\

%     $\slot$ & Execution timeslot \\
%     $\slots$ & A set of execution timeslots (execution timeline) \\

%     $\user$ & \userlong \\
%     $\users$ & A set of \userlong s \\

%     \hline
%     \end{tabular}
%     \vspace{5pt}
%     \caption{Additional notation complementing \reftbl{tbl:notation}.}
%     \label{tbl:additional_notation}
% \end{table}

% A blockchain can also be viewed as an implementation of a multi-round Validity Predicate-based Byzantine Consensus~(VPBC)~\cite{Crain18DBFT}.
% Nodes running a VPBC protocol decide on a value $\val$\footnotemark\ that satisfies a predicate $\valid()$.
% \footnotetext{To aid the discussion of \sol\ correctness guarantees we introduce additional notation summarized in \reftbl{tbl:additional_notation}}
% In the context of blockchains $\valid(\val)$ enforces structural properties such as cryptographic links between blocks, or that transactions are not malformed.
% The correctness guarantees in each round of VPBC are:
% \begin{itemize}
%     \item \textbf{VPBC-Validity} -- A non-faulty process decides on $\val$ only if a non-faulty process proposed $\val$ and if $\valid(\val)$ is true.
%     \item \textbf{VPBC-Agreement} -- No two non-faulty processes decide on different values.
%     \item \textbf{VPBC-Integrity} -- Each process decides on a value at most once.
%     \item \textbf{VPBC-Termination} -- Every non-faulty process eventually decides on a value.
% \end{itemize}
% To ensure that a VPBC protocol produces a total order of transactions, we define the predicate $\valid(\val)$ to return true if $\val$ is a non-malformed transaction and no node decides on $\val$ in any previous round.
% A VPBC protocol may also assume that node storage is stable, that each round is decided by a quorum of nodes, there is a non-zero overlap between quorums in each round, and that more than two-thirds of nodes in each round are honest.
% Under these assumptions a correct VPBC protocol satisfies blockchain correctness guarantees as
% Blockchain-Immutability is satisfied by VPBC-Integrity and the stable storage assumption,
% Blockchain-Agreement is satisfied by VPBC-Validity and VPBC-Agreement,
% finally, the persistent state guaranteed by Blockchain-Availability is satisfied by the stable storage, quorum overlap, and two-thirds honest assumptions.

% It is worthwhile to note that no consensus protocol providing validity, agreement, integrity, and termination is possible under message loss, or node failure~\cite{Akkoyunlu75TwoGenerals, Fischer85Impossibility}.
% To get around this impossibility result consensus protocols can
% deterministically reach probabilistic consensus, as in Bitcoin~\cite{Nakamoto08Bitcoin},
% or reach consensus probabilistically by guaranteeing termination if certain conditions in terms of message delivery to non-faulty processes have been met~\cite{Buchman19Tendermint, Crain18DBFT}.

% To demonstrate the correctness of \sol, we
% define its correctness guarantees in terms of VPBC validity, agreement, integrity, and termination,
% prove that the \sol\ protocol provides these properties,
% and finally map these properties to blockchain immutability, agreement, and availability.

% \subsection{\sol\ correctness guarantees}

% To define \sol's correctness guarantees we assume the execution of the \sol\ protocol can be discretized into a set $\slots$ of infitesimally small time slots.
% We also assume a set of \userlong s $\users$ and a \sol\ deployment $\zeta$.
% We define \sol's correctness guarantees as follows:
% \vspace{7pt}
% \begin{itemize}
%     \item
%     \textbf{\sol-Validity} --
%     A transaction $\tx$ can be finalized on a \sol\ blockchain only if some \userlong\ has submitted it.
%     In other words, a \sol\ user can obtain a certificate for a transaction, only if there is a user that has submitted that transaction at an earlier time.
%     Formally,
%     \[
%     \forall \user, \user' \in \users, \slot, \slot', \slot'' \in \slots,
%     \user'\!.\verify_{\slot''}(\tx) \!\rightarrow\! \cert
%     \implies
%     \user.\writef_\slot(\tx) \land \zeta.\writef_{\slot'}(\tx) \land \slot < \slot' < \slot''
%     \]

%     \todo{revise below}

%     \item
%     \textbf{Safety} -- Once $\tx$ is finalized, it will remain finalized,\footnotemark\ or
%     \[
%     (\text{\verify}(\tx) \!\rightarrow\! \cert) \implies \mathcal{G}\, (\text{\verify}(\tx) \!\rightarrow\! \cert)
%     \]
%     \footnotetext{We define the safety property using Linear Temporal Logic.}


%     \item
%     \textbf{Agreement} -- If one correct \userlong\ obtains a certificate then all correct \userlong's obtain the same certificate, or
%     \[
%     \forall \tx, \tx', \cert, \cert', (\text{\verify}(\tx) \!\rightarrow\! \cert) \land (\text{\verify}(\tx') \!\rightarrow\! \cert') \implies \tx = \tx' \land \cert = \cert'
%     \]


%     \item
%     \textbf{Liveness} -- If a process keeps resubmitting $\tx$, it will eventually become finalized, or
%     \[
%     (\text{\verify}(\tx) \!\rightarrow\! \cert) \,\mathcal{M}\, \text{\writef}(\tx)
%     \]
% \end{itemize}

% The safety property is related to the immutability property.
% While safety defines the behavior of the \verify\ function, immutability defines the behavior of data stored on the blockchain.
% The safety property is also related to availability.
% Safety implies that a user may always execute the \verify\ function, which depends on the availability of the \repsvclong.
% Note that \sol\ does not guarantee that a \userlong\ may always execute the \writef\ function to record new transactions.
% Finally, agreement in blockchains is generally understood to imply a total order over transactions.
% Since \sol\ certificates include the position of the transaction in a block on the main chain, agreement over certificates also implies agreement over order.

% \todo{revise below}


% \subsection{System model}

% To prove that \sol, as a consensus protocol, provides the aforementioned correctness guarantees, we first need to define our assumptions about the system model.
% Specifically, we assume that:

% \begin{enumerate}
% \item The instantiations of the \timesvclong, the \seqsvclong, and the \repsvclong\ do not fail permanently.
% This assumption is reasonable because the \timesvclong\ and the \repsvclong\ are themselves distributed services with uptime guarantees.
% The \seqsvclong, on the other hand, is executed in a \sol\ deployment on a single machine.
% We have a solution for a reliable replacement of a \seqsvclong\ instantiation that we will present and prove in a follow-up paper.

% \item We assume that an object replicated by the \repsvclong\ remains accessible and, specifically, that at least one correct copy of the object my be downloaded by a \userlong.
% This assumption is reasonable, because the \repsvclong\ is distributed and the objects are stored on a large number of independent nodes.
% It is therefore as unlikely that objects in the \repsvclong\ would become unavailable as it is for data to become unavailable in a network of public blockchain miners.



% \end{enumerate}



% % We proceed the correctness properties of \sol\ with a proof by invariants.
% % Invariants are predicates about a system that hold true at all points of system execution.
% % We first define a set of invariants about \sol, then prove them, and finally use the invariants to prove \sol\ correctness guarantees.

% \subsection{Safety}

% \todo{Bear pointed out a limitation of the system where we could have a collision on two timestamp attestations and we wouldn't know which one was correct. So someone could hold back an earlier one and then produce it later to move up the timestamp of a block.}

% \todo{This is an outline of the proof - needs to be made tighter after we review the correctness of the \verify\ mechanism.}

% We defined safety as
% \[
% (\text{\verify}(\tx) \!\rightarrow\! \cert) \implies \mathcal{G}\, (\text{\verify}(\tx) \!\rightarrow\! \cert).
% \]
% We assume that objects written to the \repsvclong\ cannot be erased, and so we can redefine safety as

% \begin{theorem}
% \label{thm:safety}
% \begin{align*}
% \exists\, \blocks, \times, \encls ~|~ \cert = \text{\verify}(\tx)
% \implies
% \forall\, \blocks' \supseteq \blocks, \times' \supseteq \times, \encl' \supseteq \encls,  \cert = \text{\verify}(\tx)
% \end{align*}
% \end{theorem}

% \noindent
% where once $\text{\verify}(\tx)$ returns $\cert$ based on some sets of blocks~$\blocks$, timestamp attestations~$\times$, and enclave attestations~$\encls$ it will continue to do so regardless of what objects are added to $\blocks, \times, \encls$ to form $\blocks'\!, \times'\!, \encls'$.

% \begin{proof}
% We prove \refthm{thm:safety} by induction.

% \noindent
% Base case: $\blocks' = \blocks, \times' = \times, \encls' = \encls$

% There either exist $\blocks, \times, \encls$ such that \verify\ returns a certificate, or not.
% So we can prove the base case by parts:
% \begin{itemize}
%     \item If the antecedent $\exists\, \blocks, \times, \encls ~|~ \cert = \text{\verify}(\tx)$ is true then
%     \begin{align*}
%     \exists\, \blocks, \times, \encls ~|~ \cert = \text{\verify}(\tx)
%     \implies
%     \vspace{20pt}\forall\, \blocks' \supseteq \blocks, \times' \supseteq \times, \encls' \supseteq \encls, \cert = \text{\verify}(\tx)\\
%     %
%     \top \implies \forall\, \blocks' \supseteq \blocks, \times' \supseteq \times, \encls' \supseteq \encls, \cert = \text{\verify}(\tx)
%     & &\text{by assumption}\\
%     %
%     \top \implies \forall\, \blocks, \times, \encls,  \cert = \text{\verify}(\tx)
%     & &\text{by substitution}\\
%     %
%     \top \implies \top && \text{since $\blocks, \times, \encls$ fixed}\\
%     %
%     \top
%     \end{align*}

%     \item If the antecedent $\exists\, \blocks, \times, \encls ~|~ \cert = \text{\verify}(\tx)$ is false then
%     \begin{align*}
%     \exists\, \blocks, \times, \encls ~|~ \cert = \text{\verify}(\tx)
%     \implies
%     \vspace{20pt}\forall\, \blocks' \supseteq \blocks, \times' \supseteq \times, \encls' \supseteq \encls, \cert = \text{\verify}(\tx)\\
%     %
%     \bot \implies \forall\, \blocks' \supseteq \blocks, \times' \supseteq \times, \encls' \supseteq \encls, \cert = \text{\verify}(\tx)
%     & &\text{by assumption}\\
%     %
%     \top
%     \end{align*}
% \end{itemize}

% \noindent
% Inductive hypothesis: Suppose \refthm{thm:safety} holds for some $\blocks, \times, \encls$.

% \noindent
% Inductive step: Extend $\blocks, \times, \encls$ with another object -- block, timestamp attestation, or enclave attestation.
% Formally, assume any $\blocks' \supseteq \blocks$, $\times' \supseteq \times$, and $\encls' \supseteq \encls$ and in each step let either
% $\blocks = \blocks \cup \{\block'\} \ni \block' \in \blocks'$,
% $\times = \times \cup \{\time'\} \ni \time' \in \times'$,
% or $\encls = \encls \cup \{\encl'\} \ni \encl' \in \encls'$.
% Several cases are possible:
% \begin{itemize}
%     \item The new object is a duplicate, in which case the state of $\blocks, \times, \encls$ does not change and \refthm{thm:safety} holds after the inductive step by the inductive hypothesis.

%     \item The new object does not change the set $\succs$ on line~\ref{alg:omc:succs} in \refalg{alg:omc} at any point in its execution.
%     That means that the set $\encls^*$ on line~\ref{alg:omc:auths} remains unchanged as well.
%     Consequently the calls to \path\ on line~\ref{alg:omc:path} find no fewer paths.
%     As a result the execution flow and output of \omc\ does not change, the rest of \verify\ executes without change, and \refthm{thm:safety} holds after the inductive step.

%     \item The new object, possibly in combination with objects added in previously taken inductive steps, changes the set $\succs$ on line~\ref{alg:omc:succs} in \refalg{alg:omc} at some point in its execution.
%     For the change in $\succs$ to affect the main chain, line~\ref{alg:omc:auth} would need to produce $\underline{\encl}' < \underline{\encl}$.
%     However, since $\underline{\encl}$ is already the smallest element in $\succs$ that would be a contradiction, and so \refthm{thm:safety} holds after the inductive step.
% \end{itemize}

% So, \refthm{thm:safety} holds for the inductive step and by the principle of mathematical induction \refthm{thm:safety} holds.

% \end{proof}

% \subsection{Liveness}
% \label{sec:appendix:liveness}


% % \subsection{Immutability}

% % We want to show that once a transaction $\tx$ is written onto a \sol\ blockchain, it will remain on that blockchain.
% % Specifically to the implementation of \sol, once \verify$(\tx)$ returns a certificate $\cert$, it will always return that certificate over the correct blockchain and none over any other blockchain.

% % Assumptions:
% % \begin{itemize}
% %     \item The \sol\ blockchain is comprises only main chain blocks.
% %     \item The storage used by the \repsvclong\ is stable.
% %     In other words, items replicated by the \repsvclong\ remain retrievable from storage.
% %     \item Block zero for the \sol\ blockchain is well-known.
% % \end{itemize}

% % When the \verify\ function returns \true, it means that all the checks in the process described in \refsec{sec:implementation:verify} have passed.
% % That means that storage contains sets $\blocks, \merkles, \encls$ for which \verify$(\tx)$ returns \true.
% % Since storage is stable the elements of these sets cannot be deleted from storage.
% % An attacker may, however, add additional elements to these sets, which could contain modifications.

% % verify will return true for the original combinations
% % verify will return false for any other combination

% % prove by parts:
% % - attacker adds a $\merkle'$
% % - attacker adds a $\block'$
% % - attacker adds a $\time'$
% % - attacker adds a $\encl'$



% % conclude that it will fail because one of these elements has to be added first



% % \todo{\href{https://blocky.atlassian.net/browse/BKY-2345}{BKY-2345}}

% % % Timestamp is unfakable and immutable $\leftarrow$ by CA

% % % Data has is immutable $\leftarrow$ by CA

% % % Blocks cannot be inserted post fact $\leftarrow$ \ttt{prev\_CVB\_hash} prevents us from generating blocks out of order

% % % BLOCKY is the only one that can create CVL blocks $\leftarrow$ only BLOCKY has $K_{C}^-$ with $K_{C}^+$ signed by $K_{B}^-$

% % \subsection{Agreement}



% % \todo{\href{https://blocky.atlassian.net/browse/BKY-2346}{BKY-2346}}

% % \subsection{Availability}

% % \todo{we assume that this service cannot fail}

% % \todo{\href{https://blocky.atlassian.net/browse/BKY-2348}{BKY-2348}}

% % Storage of CVBs is reliable $\leftarrow$ replication?


==> appendices/agreement.tex <==
\subsection{Agreement}
\label{sec:appendix:agreement}


==> appendices/availability.tex <==
\subsection{\sol\ Availability}
\label{sec:appendix:availability}

As mentioned earlier, a key aspect of a stable storage is its availability, or the guarantee that users can retrieve stored objects within some time bound.
The ZipperChain Replication Service encodes each object into $n_z=6$  shards including $k_z=3$ redundant shards, which means that to retrieve (and decode) an object a user must collect any $n_z - k_z = 3$ shards.
Also as mentioned earlier the availability $a_c$ guaranteed by cloud storage providers is $a_c = 99.9\%/\text{month}$.
Again, since ZipperChain objects reside on buckets in different regions, we assume independence of unavailability.
With these numbers we calculate the availability $a_z$ of a ZipperChain object as
$$
a_z = 1 - \sum_{j\, =\, n_z - k_z + 1}^{n_z} {n_z \choose j} (1-a_c)^j \,\, (a_c)^{n_z - j}
= \frac{99.999999999\%}{\text{month}},
$$
or less than $0.0003 \text{ milliseconds}$.

That number, while impressive, can be somewhat misleading.
While placing data on different buckets allows us to assume independent durability failures, the availability of data in multiple buckets may, to a degree, be plagued by same problems such as a wide-scale power outage.
So, in the worst case the unavailability of the different buckets could line up bringing $a_z$ to $99.9\% / \text{month}$.

==> appendices/durability.tex <==
\subsection{Durability}
\label{sec:appendix:durability}

\todo{copied from Colaboratory~\cite{22ZipperChainDurability} and made to compile - needs review}


We implement the ZipperChain Replication Service based on the correctness guarantees of Write Once, Read Many~(WORM) cloud storage systems.
WORM systems enable their clients to protect stored data against inadvertent modification, or deletion, to meet regulatory requirements on data retention~\cite{https://www.sec.gov/rules/interp/34-47806.htm}.
Specifically, the
AWS Simple Storage Service~(S3)~\cite{https://docs.aws.amazon.com/AmazonS3/latest/userguide/object-lock-overview.html},
Microsoft Azure Blob Storage~\cite{https://docs.microsoft.com/en-us/azure/storage/blobs/immutable-legal-hold-overview},
and Google Cloud Storage~\cite{https://cloud.google.com/storage/docs/bucket-lock}
guarantee object \emph{immutability} through legal/compliance holds on data objects that prevent anyone, including the bucket owner, from deleting or modifying objects.
Amazon~\cite{https://docs.aws.amazon.com/AmazonS3/latest/userguide/DataDurability.html},
Microsoft~\cite{https://docs.microsoft.com/en-us/azure/storage/common/storage-redundancy},
and Google~\cite{https://cloud.google.com/blog/products/storage-data-transfer/understanding-cloud-storage-11-9s-durability-target}
also design these services to provide 11 nines of \emph{durability} by replicating data across availability zones within a region.
Cloud storage providers allow, with some custom configuration, to make bucket settings publicly readable, which allows anyone to \emph{verify} that object holds are enabled.
Finally,
Amazon~\cite{https://aws.amazon.com/s3/sla/},
Microsoft~\cite{https://azure.microsoft.com/en-us/support/legal/sla/storage/v1\_5/},
and Google~\cite{https://cloud.google.com/storage/sla}
service level agreements~(SLAs) guarantee monthly 3-nines of **availability**, subject to financial penalties, which means less than 44 minutes of downtime.

\subsubsection{ZipperChain Durability On A Single Cloud Bucket}

Although the 11-nines durability guarantee is the industry standard, it is not sufficient by itself for storage of ZipperChain objects.
Let us see why.

ZipperChain stores $o = 4$ objects per block and we plan to push ZipperChain performance to the interval $i$ between blocks of $0.1$ seconds.
If we assume that we want a ZipperChain blockchain to operate for a 100 years that means that the blockchain will generate
$$
b = 100 \text{ years} \mult \frac{31536000 \text{ seconds}}{\text{year}} \mult \frac{\text{block}}{i \text{ seconds}} = 3.15\!\mult\!10^{10} \text{ blocks}
$$
blocks and $o \mult b$ objects.

For a ZipperChain to remain viable all the objects generated in each period must remain accessible.
11-nines of cloud durability allows us to define $a_c$ the annual failure rate~(AFR) of cloud objects as
$a_c = 1\!\mult\!10^{-11}$.
We transform it to a cloud object failure rate $f_c$ within a given block interval $i$ as
$$
f_c = F(a_c, i) =
a_c \frac{\text{failures}}{\text{year}} \mult
\frac{1 \text{ year}} {31536000 \text{ seconds}} \mult
\frac{i \text{ seconds}} {\text{block}}
= 3.17\!\mult\!10^{-20} \frac{\text{failures}}{\text{block}}
$$

Using the
Poisson distribution~\cite{https://en.wikipedia.org/wiki/Poisson\_distribution}
we
derive~\cite{https://github.com/Backblaze/erasure-coding-durability/blob/master/calculation.ipynb}
the probability $p_c$ of one or more failures in a period as $p_c = P(f_c) = 1 - e^{-f_c}$.
Considering that $f_c$ is very small, the difference between $p_c$ and $f_c$ is also small.
$$f_c - p_c = 5.03\!\mult\!10^{-40}$$

Finally, we calculate the cumulative durability $d^\text{*}_z$ of ZipperChain objects on a single cloud storage bucket as the probability of losing no objects created in the first period $(1-p_c)^o$, no object created in the first or second period $(1-p_c)^{2o}$, etc.
For all the periods $b$ we calculate the probability of not losing any objects as
$$
d^\text{*}_z = D^\text{*}\!(p_c, o, b) =
(1-p_c)^o \mult (1-P_C)^{2o} \mult \ldots \mult (1-P_C)^{bo} = \\
(1-p_c)^{o + 2o + \ldots + bo} =\\
(1-p_c)^{o \mult (1 + 2 + \ldots + b)} =\\
(1-p_c)^{o \mult \left((b+1) \mult \frac{b}{2}\right)} = \\
4.06\!\mult\!10^{-28}
$$
Clearly, this is woefully insufficient

\subsubsection{Cloud Storage Durability}

To understand how the ZipperChain Replication Service provides a more durable chain storage, we first must consider how cloud storage providers achieve durability.

An analysis by Backblaze~\cite{https://www.backblaze.com/blog/cloud-storage-durability/}
shows the utility of Reed-Solomon erasure codes in addressing disk failures.
They define a prototypical storage configuration with an annual disk failure rate $a_s = 0.405\%$ and a disk recovery period $r_s = 6.5\text{ days}$ based on an estimate of disk recovery rate of $12 \frac{\text{terabytes}}{\text{day}}$.
To mitigate the impact of disk failures, cloud storage providers encode an object into $n_c$ shards, including $k_c$ parity shards, and store them on independent disks.
As long as at least $n_c - k_c$ shards remain the object may be decoded.
Backblaze gives a typical configuration of $n_c=20$ and $k_c=3$.
Using the previously defined functions we calculate the probability $p_s$ of a shard being lost due to a failure of a disk as
$$
p_s = P \left( F \left(a_s, r_s \mult \frac{86400 \text{ seconds}}{\text{day}}\right)\right) = 7.21\!\mult\!10^{-5}
$$

Given the probability of a shard failing, we can use the
binomial distribution~\cite{https://en.wikipedia.org/wiki/Binomial_distribution}
probability mass function~(PMF) to calculate the probability of $k_c$ out of $n_c$ shards failing.
$$
{n_c \choose k_c} {p_s}^{k_c} \,\, (1 - p_s)^{n_c - k_c}
$$

However, an object is lost if $k_c + 1$ or more shards fail.
We calculate the joint probability of these failures using the binomial cumulative distribution function~(CDF).
$$
\text{CDF}_S = \sum_{j=k_c + 1}^{n_c} {n_c \choose j} {p_s}^j \,\, (1 - p_s)^{n_c - j}
= 1.31\!\times\!10^{-13}
$$

Finally, the durability of an object over the recovery period $r_s$ is $1 - \text{CDF}_s$ and its durability over a year is
$$
d_c = (1 - \text{CDF}_s)^{365 \frac{\text{days}}{\text{year}} / r_s \text{days} } = 0.999999999993
$$
or 11-nines.

To simplify further discussion, we define an object durability function $D(a, r, n, k)$, which aggregates the steps of the object durability calculation.

\subsubsection{ZipperChain Durability With The Replication Service}

To increase the probability that a ZipperChain chain remains viable, we apply erasure coding to ZipperChain objects to distribute their storage.
Using random linear network coding~(RLNC)~\cite{Ho2006Random}
the ZipperChain Replication Service encodes each object into $n_z = 6$ shards including $k_z = 3$ redundant shards.
We partition these shards across $n_z$ buckets located in different cloud storage providers and regions, which allows us to assume independence of bucket failures.

One key difference between the ZipperChain Replication Service and a cloud storage replication service is the time of replica recovery.
$r_s$ of $6.5 \text{ days}$ makes sense in relation to the size of a disk.
We need to define, $r_z$ based on the amount of data ZipperChain stores in each cloud bucket and the transfer rates between buckets.
The ZipperChain implementation uses $1,\!328 \text{ bytes}$
for the $o$ objects required for each block.
% <!--
% - header (block + timestamp attestation) - 1202B
% - tree - 54B
% - sequence - 32*2 + 8 = 72
% - totoal = 1202+54+72 = 1328
% -->

With the conservative assumptions that all $ob$ objects generated over the 100 years of operation exist in year one and with a conservative one-connection estimate of inter-region transfer speed~\cite{https://medium.com/slalom-technology/examining-cross-region-communication-speeds-in-aws-9a0bee31984f}
is $160 \text{ Mbps}$
we calculate the time $r_z$ to recover the state of a bucket user by ZipperChain as
$$
r_z = 1328 \frac{\text{bytes}}{\text{block}}
\mult \frac{\text{block}}{o \text{ objects}}
\mult \frac{b \text{ objects}}{(n_z - k_z) \text{ buckets}}
\mult 8 \frac{\text{bits}}{\text{byte}}
\mult \frac{1 \text{Mb}}{ 1\!\mult\!10^6 \text{ bits}}
\mult \frac{1 \text{ second}}{ 160 \text{ Mb}}
= 1.74\!\mult\!10^5 \frac{\text{seconds}}{\text{bucket}}
$$
or about $48 \text{ hours}$.

Given these constants, we calculate the durability $d_z$ of a ZipperChain object as
$$
d_z = D(1-d_c, r_z, n_z, k_z) \implies 35 \text{ nines}
$$

The 35-nines of object reliability achieved by the ZipperChain Replication service is a marked improvement over the 11-nines of cloud storage reliability.
But how do 35-nines of object durability translate to the probability that a ZipperChain chain remains viable over a 100 year period?

To answer that question we use the cumulative durability function $D^\text{*}$.
Plugging in the probability of object failure $1 - d_z$, the number of ZipperChain objects $o$ created for each block, and the number of $b$ we get
$$
d^\text{*}_z = 0.9999999999999903
$$
or 14-nines of cumulative durability.

Thus with the ZipperChain Replication Service our users may trust that the ZipperChain chain retains \emph{durability}, because with high probability its objects will not be lost through disk, or storage provider failure.
Users may also \emph{verify} through exposed cloud service configurations the level of replication and that each bucket has legal/compliance holds enabled to guarantee object \emph{immutability}.

==> appendices/immutability.tex <==
\subsection{Immutability}
\label{sec:appendix:immutability}

\begin{definition}[Identifies]
Given the identification operator `$\,\ids\,$' and two data structures $x$ and $y$, $x \ids y \iff$ $x$ contains a reference to $y$.
\end{definition}
\noindent
Without loss of generality, if $y$ is a member of $x$ then $x$ \emph{identifies} the value of $y$, or in other words $x.y \implies x \ids y$.


\begin{definition}[Hashes]
Given the hashing operator `$\,\,\hashes\,$' and two data structures $x$ and $y$, $x \hashes y \iff x \ids \hash(y)$.
\end{definition}

\begin{definition}[Signs]
Given the signing operator `$\,\,\signs\,$' and two data structures $x$ and $y$, $x \!\!\underset{K}{\signs}\!\! y \iff x \ids \encrypt{K^-}{\hash(y)}$.
For convenience, the underset key may be omitted. 
\end{definition}


\begin{theorem}
    Given,
        a set $\zpr$ of on main chain triads,
        \timesvclong\ public key $\key^+_\timesvc$,
        \seqsvclong\ public key $\key^+_\seqsvc$,
    the hash and order of a transaction $\tx \in \zpr$ remains signed by the \timesvclong\ private key $\key^-_\timesvc$ and by the \seqsvclong\ private key $\key^-_\seqsvc$.
\end{theorem}

\begin{proof}
We will show by induction ...

Base case:

Let $\tri_0 = \zpr[0]$.
Since $\tri_0$ is part of \omc\ output, we know that $\tri_0$ is a true triad.
In a true triad $\time \signs \block$, $\seq \uids \block$, and $\seq \usigns \time$.


Let $\tri$ be true triad $\langle \block, \time, \seq \rangle$.
By the construction of $\time$ we know that $\time \signs \block$.
Similarly, we know by the construction of $\seq$ that $\seq \uids \block$ and $\seq \usigns \time$.
$a \uhashes b$

From the construction process of blocks, we know that there is a one to one relationship between
\end{proof}

==> images/write.tex <==
\begin{tikzpicture}[node distance=2cm]
\node (user) [process] {\userlong};
\node (batchit) [process, below of=user] {\batchit};
\node (zipit) [process, below of=batchit] {\zipit};
\node (timestampit) [process, right=2.1cm of zipit] {\makecell[c]{Timestamp\\Service}};
\node (storeit) [process, below of=zipit] {\storeit};
\node (replicateit) [process, left=1.9cm of storeit] {\makecell[c]{Replication\\Service}};
\node (sequenceit) [process, right=2.1cm of storeit] {\makecell[c]{Sequencer\\Service}};
% \node (cacheit) [process, below of=storeit] {CacheIt};
% \node (database) [process, below of=cacheit] {Database};

\draw [farrow] (user) -- node[anchor=west] {\ref{step:write:user->batchit}~$\tx$} (batchit);

% \draw let \p1 = (b), \p2 = (bp), \p3 = (t-1) in
% (\x3,\y2*0.5+\y1*0.5) node [seq_block] (s-1) [anchor=center] {$\seq_{\idxk-1}$};

\draw let \p1 = (batchit), \p2 = (replicateit) in
(\x2, \y1) node (br) [anchor=center] {};
\draw [farrow] (batchit) 
-- node[anchor=south] {\ref{step:write:batchit->replication}~$\merkle$} (br.center)
-- (replicateit)
;

\draw [farrow] (batchit) 
-- node[anchor=west] {\ref{step:write:batchit->zipit}~$\langle \hash(\merkle), \merkle.\uuid \rangle$} 
(zipit)
;


% \draw let \p1 = (replicateit), \p2 = (zipit) in
% (\x1,\y2) node (a1) [anchor=center] {};
% \draw [farrow] (replicateit.north) 
% -- (a1.center) 
% -- node[anchor=south] {\ref{step:write:replication->zipit}~$\encl\texttt{[]}$} (zipit);

\draw [darrow] (zipit) -- 
node[anchor=south] {\ref{step:write:zipit->attest}~$\langle \hash(\block), \block.\time^\uuid \rangle$} 
node[anchor=north] {$\time$} 
(timestampit);

\draw [farrow] (zipit) -- 
node[anchor=west] {\ref{step:write:zipit->storeit}~$\langle \block, \time \rangle$} 
(storeit);

\draw [farrow] 
([yshift=0.25cm]storeit.west) 
-- 
node[anchor=south] {\ref{step:write:storeit->replication}~$\langle \block, \time \rangle$} 
([yshift=0.25cm]replicateit.east);

\draw [darrow] 
([yshift=0.0cm]storeit.east) 
-- 
node[anchor=south] {\ref{step:write:storeit->seq}~$\langle \hash(\time), \time.\uuid \rangle$} 
node[anchor=north] {$\seq$} 
([yshift=0.0cm]sequenceit.west);

\draw [farrow] 
([yshift=-0.25cm]storeit.west) 
-- 
node[anchor=north] {\ref{step:write:seq->replication}~$\seq$} 
([yshift=-0.25cm]replicateit.east);

% \draw [farrow] (storeit) -- 
% node[anchor=east] {\ref{step:write:storeit->cacheit}~$\langle \batch, \merkle, \block, \time, \seq \rangle$} 
% (cacheit);

% \draw [farrow] (cacheit) -- 
% node[anchor=east] {\ref{step:write:cacheit->database}~$\forall \tx \in \merkle, \tx \mapsto \langle \merkle, \block, \time, \seq \rangle$} 
% (database);


\node (ctrl1) [below=0.5cm of storeit, anchor=center] {};
\node (ctrl2) [below right=0.5cm and 4.1cm of storeit, anchor=center] {}; 
\node (ctrl3) [right=4.1cm of batchit, anchor=center] {}; 
\draw[farrow] (storeit) 
-- (ctrl1.center) 
-- node [anchor=north] {\ref{step:write:storeit->batchit}~$\merkle.\uuid$} (ctrl2.center)
-- (ctrl3.center)
-- (batchit)
;


% -- node [anchor=south] {\ref{step:write:cacheit->batchit}~$\batch$} (ctrl1) -- (ctrl2.east) -- (batchit);

\end{tikzpicture}

% \begin{sequencediagram}
%     % \tikzstyle{inststyle}+=[bottom color=white, top color=white, ]

%         \newthread[white]{u}{\userlong}
%         \newthread[white]{b}{\batchit}
%         \newthread[white]{z}{\zipit}
%         \newinst[0.25]{t}{\makecell[c]{Timestamp\\Service}}
%         \newinst[0.25]{s}{\storeit} 
%         \newinst[0.25]{r}{\makecell[c]{Replication\\Service}} 
%         \newinst[0.25]{q}{\makecell[c]{Sequencer\\Service}} 
        
%         \begin{call}
%             {u}{\ref{step:write:user->batchit}~$\tx$}
%             {b}{}
%         \end{call}
        
%         \begin{call}
%             {z}{}
%             {r}{$[\encl]$}
%         \end{call}
        
%         \begin{call}
%             {z}{}
%             {b}{$\langle \batch, \merkle \rangle$}
%         \end{call}
        
%         \begin{call}
%             {z}{$\hash(\block)$}
%             {t}{$\time$}
%         \end{call}
        
%         \begin{messcall}
%             {z}{$\langle \batch, \merkle, \block, \time \rangle$}
%             {s}
            
%             \begin{call}
%             {s}{$\langle \merkle, \block, \time \rangle$}
%             {r}{}
%             \end{call}
            
%             \begin{call}
%             {s}{$\block.\uuid$}
%             {q}{$\encl$}
%             \end{call}
            
%             \begin{call}
%             {s}{$\encl$}
%             {r}{}
%             \end{call}
            
%             \mess{s}{$\batch$}{b}
%             % \begin{messcall}
%             % {s}{$\batch$}{b}
%             % \end{messcall}
%         \end{messcall}
        
        
        
        
        
         
        
        
        
%         % \mess{b}{$\langle \batch, \merkle \rangle$}{z}
        
        
%         % \mess{b}{$\langle \batch, \merkle \rangle$}{z}

%         % \begin{call}
%         %     {b}{$\langle \batch, \merkle \rangle$}
%         %     {z}{Handshake}
%         % \end{call}

%         % \stepcounter{seqlevel}
%         % \begin{call}
%         %     {c}{ws.connect}
%         %     {s}{ws.connectes}
%         % \end{call}

%         % \stepcounter{seqlevel}
%         % \mess{c}{ws.message}{s}
%         % \mess{s}{ws.message}{c}
%         % \mess{c}{ws.message}{s}

% \end{sequencediagram}
